Synthetic Polarization Maps of an Outflow Zone from Magnetohydrodynamic Simulations

The canonical theory of star formation in a magnetized environment predicts the formation of hourglass-shaped magnetic fields during the prestellar collapse phase. In protostellar cores, recent observations reveal complex and strongly distorted magnetic fields in the inner regions that are sculpted by rotation and outflows. We conduct resistive, nonideal magnetohydrodynamic (MHD) simulations of a protostellar core and employ the radiative transfer code POLARIS to produce synthetic polarization segment maps. Comparison of our mock-polarization maps based on the toroidal-dominated magnetic field in the outflow zone with the observed polarization vectors of SiO lines in Orion Source I shows a reasonable agreement when the magnetic axis is tilted at an angle $\theta = 15^{\circ}$ with respect to the plane-of-sky and if the SiO lines have a net polarization parallel to the local magnetic field. Although the observed polarization is from SiO lines and our synthetic maps are due to polarized dust emission, a comparison is useful and allows us to resolve the ambiguity of whether the line polarization is parallel or perpendicular to the local magnetic field direction.

==> MM.tex <==
\input{top-apj}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
%%\newcommand{\micro}{\upmu }
% Headers for odd and even pages, respectively:
\shorttitle{Synthetic Polarization maps}
% If more than two authors, use {\em et al.}
\shortauthors{Bino et al.}
\newcommand{\cc}{\,{\rm cm}^{-3} } 

\begin{document}

\title{Synthetic Polarization Maps from Resistive Magnetohydrodynamic Simulations}

%% AUTHOR/INSTITUTIONS FOR AASTEX6.1:
\author{Gianfranco Bino}
\affiliation{Department of Applied Mathematics, Western University, London, ON, N6A 5B7, Canada.}


\author{Shantanu Basu}
\affiliation{Department of Applied Mathematics, Western University, London, ON, N6A 5B7, Canada.}
\affiliation{Department of Physics \& Astronomy, Western University, London, ON, N6A 3K7, Canada.}

\author{Masahiro Machida}
\affiliation{Department of Earth and Planetary Sciences, Faculty of Sciences, Kyushu University, Fukuyoka, Fukuyoka  819-0395, Japan.}
\affiliation{Department of Physics \& Astronomy, Western University, London, ON, N6A 3K7, Canada.}


%% AUTHOR/INSTITUTIONS FOR EMULATE APJ:
% \author{Patricio~E.~Cubillos\altaffilmark{1,2},
% Joseph~Harrington\altaffilmark{1},
% and
% Third~Author\altaffilmark{1}
% }
% \affil{\sp{1} Planetary Sciences Group, Department of
%               Physics, University of Central Florida, Orlando, FL 32816-2385\\
%        \sp{2} Space Research Institute, Austrian Academy of Sciences,
%               Schmiedlstrasse 6, A-8042, Graz, Austria}

\email{gbino@uwo.ca}
\email{basu@uwo.ca}
\email{machida.masahiro.018@m.kyushu-u.ac.jp}
% %% Extra info for aastex:
% \received{Yesterday}
% \revised{Today}
% \accepted{Tonight}
% \published{Tomorrow}
% \submitjournal{AASJournal}

\begin{abstract}
We aim to study the evolution of stellar objects in the early protostellar phase. In order to accurately model the dense, star forming regions of protostellar cores, non-ideal magnetohydrodynamic (MHD) simulations are used by solving the resistive MHD equations on a nested grid at a series of length scales. The simulations are used to study three instances in time for the core's evolution represented in terms of the core's mass. This methodology enables us to resolve the central protostellar region on small scales.
%% and is more computationally efficient than the adaptive grid method. 
In doing such, we take our MHD model as an input to the radiative transfer code, POLARIS used to simulate synthetic polarization maps at all length scales within the core allowing for robust, high resolution outputs of the polarization segments within the small scale regions of the core. Additionally, these synthetic polarization maps are used to model the magnetic field and polarization state of Orion Source I \citep{hir2020}. Through superimposition and an analysis on the mean field direction, we infer the emission and absorption properties of the ALMA measurements from both the POLARIS and MHD simulations.
\end{abstract}

% http://journals.aas.org/authors/keywords2013.html
\keywords{stars: formation --- ISM: magnetic fields --- mathematical model}


\section{Introduction}
\label{introduction}
{\bf
Magnetic field plays an important role in the star formation process. 
The configuration of  magnetic fields (or magnetic field vectors) in star-forming cores can be expected by polarization observation which has been done in various star-forming regions.
The observed polarization vectors (or segments) are either  parallel or perpendicular to the magnetic field vectors, depending on the observation method (dust thermal emission,  dust extinction and  line emission). 
Recent polarization observations indicate that magnetic fields in prestellar and protostellar cores  are well aligned in any scale \citep{girart06,girart09, PC16, ching16, alves18,maury18,lee18}, indicating that the star-formation process is regulated by the magnetic field (or Lorentz force), not by turbulence. 
Especially, the configuration of the magnetic field in a small scale of $<100-1000$\,au is crucially important for understanding the disk formation and outflow driving. 

One of the most interesting target in observations is Orion Source I located in the nearest high-mass star forming region Orion KL (418\,pc)  in the Orion nebula.
For the object,  a nearly edge-on disk with a size of $\sim50$\,au has been observed.
Thus, Orion Source I is a suitable object for observing the  disk and outflow.
Recently, \citet{hirota17} confirmed the rotation of molecular outflow, in addition to the rotation of the disk. 
Then, using the Bernoulli's theorem and the angular momentum conservation law, they estimated the outflow launching radius as $\sim5-25$\,au, indicating that the molecular outflow is directly driven from the disk surface, not entrained by an unseen high-velocity jet. 
The rotation of molecular outflow has been observed  also in recent other ALMA observations \citep{bjerkeli16,tabone17,zhang18}.

Very recently, \citet{hir2020} observed the polarized emission within the outflow of Orion Source I.
In the observation, the polarization vectors are well aligned, while they are neither parallel to perpendicular to the outflow axis or the propagation direction of the outflow. 
Since the polarization vectors are considered to be produced  by the projected and integrated magnetic fields, it is difficult to image the actual configuration (or three dimensional configuration) of the magnetic field. 
Thus, synthetic observation or synthetic polarization map is necessary to understand the configuration of the magnetic field. 

The synthetic observation using the core collapse simulation is very useful to untangle the complex polarization observations and relate the polarization vectors to magnetic vectors. 
The first such study was carried out by  \citet{tomisaka11}.
He made the polarization maps from his two-dimensional ideal MHD core collapse simulations. 
In his study, the polarization degree and pattern before and after the first core formation were discussed. 

\citet{reissl17} also executed the synthetic observation using the data of a core collapse simulation. 
In their study, since they focused on the dust alignment mechanism, their simulation data (or core collapse simulation) is not realistic.
In their simulation, they cannot correctly resolve the disk and outflow driving region because a considerably large-sized sink (12.6\,au) was imposed \citep{machida14,hennebelle20}. 
In addition, the magnetic field strength adopted in their simulation is as weak as $\mu=26$, where $\mu$ is the mass-to-flux ratio normalized by the critical value. 
With such a very weak magnetic field, a different mode of outflow appears with ideal MHD simulation, as shown in \citet{tomisaka02}.
In addition, it is difficult to compare past synthetic observations with the observations at ALMA era because the  spatial resolution of the polarization maps in \citet{tomisaka11} and \citet{reissl17} are not sufficient.

This study aim to investigate the polarization pattern in a small scale around the disk and outflow driving region.
Firstly, we execute a high-resolution core collapse simulation using our nested grid code.
Then, we solve the radiative transfer and make polarization maps. 
Finally, we compare the polarization maps between our synthetic observation and observation of Orion Source I, in order to understand the configuration of magnetic field around the outflow driving region.
The structure of this paper is as follows. 

}

\section{Methods}
\subsection{Magnetohydrodynamic Simulations}
In order to simulate the dense, star-forming core of molecular clouds, non-ideal magnetohydrodynamic  simulations are used as the basis for our model. 
{\bf
In this subsection, we explain the settings of our simulation.

As the initial state, we prepare the prestellar core with a Bonnor-Ebert density profile that is constructed with a central density  $6\times10^5\cc$ and an isothermal temperature $10$\,K.
The mass $M_{\rm cl}$ and radius $R_{\rm cl}$ of the initial core are $M_{\rm cl} = 2M_{\odot}$ and $R_{\rm cl} = 1.2\times10^4$\,au, respectively. 
Note that the cloud density is enhanced by a factor of $f$ ($f=1.68$) to promote the contraction \citep{machida20}.  
A uniform magnetic field $B_0=3.2\times10^{-5}$\,G and a rigid rotation $\Omega_0=1.3\times10^{-13}$\,s$^{-1}$ are adopted to the initial core, in which the rotation axis is parallel to the magnetic field.
For the initial core, the mass-to-flux ratio normalized by the critical value $1/(2\pi G^{1/2})$ is $\mu_0=2$. 
The ratio of thermal $\alpha_0$ and rotational $\beta_0$ energy to gravitational energy are $\alpha_0=0.42$ and $\beta=0.024$, respectively. 
}

In these dense regions, the clouds are lightly ionized and because of this the magnetic field cannot be coupled to the neutral material and so the flux frozen property is no longer valid. In doing so, we solve the resistive MHD equations including self-gravity:
\begin{flalign}
&\frac{\partial \rho}{\partial t} + \nabla \cdot (\rho \textit{\textbf{v}}) = 0, \\
&\rho \frac{\partial \textit{\textbf{v}}}{\partial t} + \rho(\textit{\textbf{v}} \cdot \nabla)\textit{\textbf{v}} = -\nabla p + \textit{\textbf{j}} \times \textit{\textbf{B}} - \rho  \nabla \Phi, \\
&\frac{\partial \textit{\textbf{B}}}{\partial t} = \nabla \times (\textit{\textbf{v}} \times \textit{\textbf{B}}) + \eta \nabla^2 \textit{\textbf{B}}, \\
&\nabla^2 \Phi = 4\pi G \rho.
\end{flalign}
We simulate the core evolution on a nested grid \citep{mats2003,machida04,machida13} for 13 levels up to $t \approx 89547$ years corresponding to a prestellar mass of $M \approx 0.3M_{\odot}$. 
{\bf 
For the simulation, the box size and cell width of the first level of grid ($l=1$) are $3.7 \times 10^5$\,au and $5.9 \times 10^3$\,au, while those for the most finest grid ($l=13$) are 92\,au and 1.44\,au, respectively. 
We impose a sink cell to accelerate the calculation, in which the sink threshold density $10^{12}\cc$ and sink accretion radius $r_{\rm sink}=2$\,au are adopted. 
}
Our study will pertain to three instances in the evolutionary period when the core achieves a mass of  $M = 0.01M_{\odot}$,  $ 0.2M_{\odot}$ and $ 0.28M_{\odot}$. 

\subsection{Radiative Transfer Simulations}
In order to simulate synthetic polarization maps, we use the POLARIS code \citep{rei16} which solves the three dimensional radiative transfer problem
\begin{align}
    \frac{{\rm d} \textit{\textbf{S}} }{ {\rm d} l } = -\hat{\textit{\textbf{R}}}(\alpha )\hat{\textit{\textbf{K}}} \hat{\textit{\textbf{R}}}(\alpha)^{-1}\textit{\textbf{S}} + \textit{\textbf{J}}
\end{align}
 for all Stokes parameters contained in the Stokes four-vector $\textit{\textbf{S}} = \left[ I, Q, U, V \right]^{\top}$ (for $I$, $Q$, $U$ and $V$ representing the total intensity, the states of linear polarization and circular polarization respectively). Here, $\hat{\textit{\textbf{R}}}(\alpha )$ is the rotation matrix, $\hat{\textit{\textbf{K}}}$ is the Muller matrix which describes extinction, absorption and scattering and $\textit{\textbf{J}}$ is the energy transfer contribution due to emission. We refer the reader to the \href{https://www1.astrophysik.uni-kiel.de/~polaris/content/manual.pdf}{software manual} for further details. We model the density, temperature, velocity and magnetic field profiles directly from the MHD simulations. Additionally, we assume dust grains are non-spherical with a grain size following a power-law distribution \citep{mat77} for a minimum size $a_{\rm min} = 0.005 \micro \rm m $ and a maximum size $a_{\rm max} = 2 \micro \rm m $. The dust to gas mass ratio is 0.01 and the grain alignment is taken to follow the Davis-Greenstein (DG) alignment mechanism \citep{DG1951}. We adopt a T-Tauri like star as our model's radiation source positioned at the center of the simulation grid with $R = 0.9 R_{\odot}$ and $T = 4000$K.

\begin{figure*}
\centering
  \includegraphics[width=\textwidth]{mhd_dens_vel.pdf}
  \caption{The number density taken along $x = 0$ overlaid with the velocity vectors resulting from the MHD simulation. From left to right each panel is representative of $M = 0.01M_{\odot}$,  $= 0.2M_{\odot}$ and $= 0.28M_{\odot}$.} 
\label{mag_dens}
\end{figure*} 

 \begin{figure*}
\centering
  \includegraphics[width=1\textwidth]{mhd_mag_3d.pdf}
  \caption{Three dimensional renderings of the MHD simulation output taken about the surface of the disk. From left to right each panel is representative of $M = 0.01M_{\odot}$,  $= 0.2M_{\odot}$ and $= 0.28M_{\odot}$.
{\bf
In each panel, magnetic field lines (blue lines) and high-density region (orange surface) are plotted. 
The box size (185\,au) is the same among three panels.  
}
} 
\label{mag_3d}
\end{figure*}
\section{Results}
\subsection{Simulatoin Results}
In Figure \ref{mag_dens}, we provide a plot along $x = 0$ of the density overlaid with the directional velocity field vectors in all instances in the core's evolutionary period. Furthermore, in Figure \ref{mag_3d} the three dimensional renderings of the magnetic field are also given about the disk's surface.
{\bf
In the simulation, the outflow is driven by the rotationally supported disk. 
We can confirm the whole region of the outflow in the left panel of Figure~\ref{mag_dens}.
The size of the outflow at this epoch is about 180\,au. 
Then, the outflow extends up to $\sim3\times10^5$\,au by the end of the simulation. 
In Figure~\ref{mag_dens}, the central yellow region corresponds to the rotationally supported disk which is enclosed by the pseudo disk colored by orange and purple. 
The rotationally supported disk gradually grows and has a radius of $\sim30$\,au when the protostellar mass reaches $0.28 M_{\odot}$ (right panel of Fig.~\ref{mag_dens}). 
The middle and right panel of Figure~\ref{mag_dens} indicate that the outflow is mainly driven by the region near the outer edge of the rotationally supported disk as seen in a recent ALMA observation \citep{alves17}.

The left panel of Figure~\ref{mag_3d} indicates that the configuration of the magnetic field lines is composed of two components. 
The magnetic field lines are strongly twisted within the outflow, while they are radial configuration outside the outflow (compare left panels of Fig.~\ref{mag_dens} and Fig.~\ref{mag_3d}). 
The middle and right panels of Figure~\ref{mag_3d} indicate that the configuration of the magnetic field lines near the protostar and disk change over time. 
}



\subsection{POLARIS Output}
We run our radiative transfer simulations for all three instances in the core's evolution at a series of declination angles. The declination angles are taken to tilt in the direction of the observer at $\theta \in [0 , \pi/6, \pi/4, \pi/3, \pi/2 ] $. Our outputs are given in Figures \ref{m01}, \ref{m02} and \ref{m03} for $M = 0.01M_{\odot}$,  $= 0.2M_{\odot}$ and $= 0.28M_{\odot}$ at level $L = 12$. POLARIS will output the polarization that results from the integrated scattering and emission properties of the dust grains and their orientation is perpendicular to the local magnetic field. In order better gauge what the inferred magnetic field is, we have rotated the vectors in Figures \ref{m01}, \ref{m02} and \ref{m03} by 90 degrees so that they are now assumed to have parallel alignment to the magnetic field.
\subsection{ALMA Data}
\cite{hir2020} probed the magnetic field in the bipolar outflow region of a high mass protostar from Orion Source I (SrcI). Polarization measurements of the SiO rotational transitions were observed using ALMA on October 12$^{\text{th}}$ and 17$^{\text{th}}$ 2017 \citep{hir2020}.
They estimate the magnetic field strength in the outflow lobe to be approximately 30 mG using the Davis-Chandresekhar-Fermi method and suggest the configuration being either toroidal or poloidal depending on how the polarization vectors are oriented relative to the magnetic field. We aim to further probe the magnetic field structure and provide insight as to how the polarization vectors may be oriented with respect to the local magnetic field. By matching the length scales of the POLARIS outputs, the synthetic polarization maps can be used to model the polarization state and the magnetic field of Orion Source I.  We find the level 10 POLARIS simulations best match the length scale of the ALMA data and we present an overlay of the polarization segments in Figures \ref{alma_pol_1}, \ref{alma_pol_2} and \ref{alma_pol_3} for all three instances. If the polarization measurements of the ALMA data are given from emission, we expect them to be oriented perpendicular to the local magnetic field. Otherwise if the measurements given from absorption, the segments will be oriented parallel to the local magnetic field. Thus, in Figures \ref{alma_pol_1}, \ref{alma_pol_2} and \ref{alma_pol_3}, we can infer whether the measurements are from emission or absorption by assessing the ALMA data with the POLARIS output. In our simulations we had rotated the polarization vectors from the POLARIS outputs by 90 degrees to infer the magnetic field and so if the alignment of the ALMA data is parallel to the POLARIS output, we infer the measurements result from absorption whereas if the data is oriented perpendicular to the POLARIS outputs then we infer emission measurements. In order to assess the alignment quantitatively, we compute the mean offset angle that the magnetic field makes with the $z-$axis from both the MHD and POLARIS simulations. We define the quantity
\begin{align}
    \Delta \phi^{(L)} = |\hat{\phi} - \phi^{(L)}|,
\end{align}
as the absolute residual between the mean offset angle of the ALMA data $\hat{\phi}$, and the simulation output at a given level $L$, $\phi^{(L)}$. Here, $\hat{\phi}$ is estimated under the assumption that the polarization segments are aligned with the local magnetic field. Thus, for $L = 10$, we compute:
\begin{flalign*}
&\Delta \phi_{\text{M}}^{(10)}  = 46.91 \; \text{deg}, \; \;  \Delta \phi_{\text{P}} ^{(10)}= 52.89 \; \text{deg} \; \; \text{for} \; \; M = 0.01M_{\odot}, \\
&\Delta \phi_{\text{M}}^{(10)}  = 1.78 \; \text{deg}, \quad  \Delta \phi_{\text{P}}^{(10)} = 2.52 \; \text{deg} \quad \text{for} \; \; M = 0.2M_{\odot}, \\
&\Delta \phi_{\text{M}}^{(10)}  = 1.37 \; \text{deg}, \quad  \Delta \phi_{\text{P}}^{(10)} = 5.49 \; \text{deg} \quad \text{for} \; \; M = 0.28M_{\odot},
\end{flalign*}
where the subscripts 'M' and 'P' are representative of the MHD and POLARIS simulations respectively. Furthermore, we demonstrate in Figure \ref{alma_comp} the mean misalignment for each instance at each simulation level. Additionally, we include the mean misalignment of the ALMA data under the assumption of parallel magnetic field alignment (red $\times$ mark) and perpendicular alignment (violet $\times$ mark). Visually, the calculations suggest the ALMA data is best modelled by the instances having $M = 0.2M_{\odot}$ and $ M = 0.28M_{\odot}$ with polarization segments being aligned parallel to the local magnetic field. By this, we infer that the polarization measurements result from absorption rather than emission. If we compare these assessments with our calculations of $\Delta \phi^{(10)}$, we see that the POLARIS outputs for $M = 0.2M_{\odot}$ have the smallest residual and so we estimate that the core is best modelled by this stage in the protostellar evolution.

\section{Discussion}

\begin{figure*}
\centering
%%  \includegraphics[width=1\textwidth]{M001_2.pdf}
  \caption{Synthetic polarization maps for the instance $M = 0.01M_{\odot}$ given at $L = 12$. The figures are given at a series of declination angles $\theta$ representative of tilting the system toward the direction of the observer. The polarization segments have been rotated by 90 degrees to be representative of the inferred local magnetic field.} 
\label{m01}
\end{figure*} 

\begin{figure*}
\centering
%% \includegraphics[width=1\textwidth]{M02_2.pdf}
  \caption{Synthetic polarization maps for the instance $M = 0.2M_{\odot}$ given at $L = 12$. The figures are given at a series of declination angles $\theta$ representative of tilting the system toward the direction of the observer. The polarization segments have been rotated by 90 degrees to be representative of the inferred local magnetic field.} 
\label{m02}
\end{figure*}

\begin{figure*}
\centering
%%  \includegraphics[width=1\textwidth]{M028_2.pdf}
  \caption{Synthetic polarization maps for the instance $M = 0.28M_{\odot}$ given at $L = 12$. The figures are given at a series of declination angles $\theta$ representative of tilting the system toward the direction of the observer. The polarization segments have been rotated by 90 degrees to be representative of the inferred local magnetic field.} 
\label{m03}
\end{figure*}

\begin{figure*}
\centering
%%  \includegraphics[width=\textwidth]{Paper/M001_1.pdf}
  \caption{The polarization segments of the ALMA data (bold vectors) overlaid with the simulated synthetic polarization maps from POLARIS where the dust grains are assumed to have parallel alignment to the local magnetic field. The figures are given for $M = 0.01M_{\odot}$ at $L = 10$ where the declination angle $\theta$ is taken toward the observer. } 
\label{alma_pol_1}
\end{figure*}

\begin{figure*}
\centering
%%  \includegraphics[width=1\textwidth]{Paper/M02_1.pdf}
  \caption{The polarization segments of the ALMA data (bold vectors) overlaid with the simulated synthetic polarization maps from POLARIS where the dust grains are assumed to have parallel alignment to the local magnetic field. The figures are given for $M = 0.2M_{\odot}$ at $L = 10$ where the declination angle $\theta$ is taken toward the observer. } 
\label{alma_pol_2}
\end{figure*}

\begin{figure*}
\centering
 %% \includegraphics[width=1\textwidth]{Paper/M028_1.pdf}
  \caption{The polarization segments of the ALMA data (bold vectors) overlaid with the simulated synthetic polarization maps from POLARIS where the dust grains are assumed to have parallel alignment to the local magnetic field. The figures are given for $M = 0.28M_{\odot}$ at $L = 10$ where the declination angle $\theta$ is taken toward the observer. } 
\label{alma_pol_3}
\end{figure*}

\begin{figure*}
\centering
%%  \includegraphics[width=\textwidth]{Paper/align.pdf}
  \caption{The mean offset angle that the magnetic field makes with the $z-$axis at each level in the MHD simulation (green), the POLARIS simulation (blue) and the misalignment between the MHD and POLARIS simulations (dotted black). The red $\times$ mark is the mean offset angle of the implied magnetic field for the ALMA data assuming parallel alignment and the violet $\times$ mark assumes perpendicular alignment. From left to right: $M = 0.01M_{\odot}$, $M = 0.2M_{\odot}$, $M = 0.28M_{\odot}$} 
\label{alma_comp}
\end{figure*}

\section{Conclusion}
\label{Conclusion}
\bibliography{templateMM}{}
\bibliographystyle{aasjournal}
\end{document}

